K-CIRCT: A Layered, Composable, and Executable Formal Semantics for CIRCT Hardware IRs

CIRCT, an open-source EDA framework akin to LLVM for software, is a foundation for various hardware description languages. Despite its crucial role, CIRCT's lack of formal semantics challenges necessary rigorous hardware verification. Thus, this paper introduces K-CIRCT, the first formal semantics in {\K} for a substantial CIRCT subset adequate for simulating a RISC-V processor. Our semantics are structured into multiple layers: (1) MLIR static semantics, which covers fundamental MLIR concepts across domains; (2) CIRCT common semantics, featuring a generic hardware model that captures key hardware features across dialects; and (3) composable and extensible semantics for specific dialects, formalized individually using a unified approach. This approach has been applied to formalize CIRCT core dialects. We validated our semantics through full-rule coverage tests and assessed its practicality using the popular RISC-V hardware design, riscv-mini.

==> lib/custom.tex <==
\newcommand{\cell}[2]{\langle #1 \rangle #2 \langle/ #1 \rangle}

==> lib/jstyle.tex <==




\usepackage{tabularx,longtable,ltablex,multirow,booktabs,xcolor,colortbl,pifont}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{subcaption}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{listings}
\usepackage{tabularx}

\definecolor{hgreen}{HTML}{8CB26E}
\definecolor{mgreen}{HTML}{A9C695}
\definecolor{lgreen}{HTML}{D9E7D6}
\definecolor{hred}{HTML}{AC5A54}
\definecolor{mred}{HTML}{DCADA9}
\definecolor{lred}{HTML}{F1D0CD}
\definecolor{hblue}{HTML}{738DBB}
\definecolor{mblue}{HTML}{98ADD1}
\definecolor{lblue}{HTML}{DDE8FA}
\definecolor{hgray}{HTML}{585858}
\definecolor{mgray}{HTML}{BCBCBC}
\definecolor{lgray}{HTML}{F0F0F0}
\definecolor{hyel}{HTML}{D1B765}
\definecolor{myel}{HTML}{EEDDAA}
\definecolor{lyel}{HTML}{FDF2D0}
\definecolor{hpur}{HTML}{9174A3}
\definecolor{mpur}{HTML}{C4B3CE}
\definecolor{lpur}{HTML}{DFD5E6}
\definecolor{myhgreen}{RGB}{0,102,0}

\newcommand{\jbox}[1]{\begin{center}\begin{tikzpicture}\node[draw, fill=white, text width=7cm, inner sep=3pt, align=left, inner xsep=7pt] at (0,0) {\textit{#1}};\end{tikzpicture}\end{center}}


\newif\ifshowcomments
\showcommentstrue

\ifshowcomments
\newcommand{\yao}[1]{\mytodoblue{[yao: #1]}}
\newcommand{\hong}[1]{\mytodoorange{[hong: #1]}}
\else
\newcommand{\yao}[1]{}
\newcommand{\hong}[1]{}
\fi



\newcommand{\mytodoblue}[1]{\textcolor{blue}{\ding{46}~{\sf}~#1}}
\newcommand{\mytodored}[1]{\textcolor{red}{\ding{46}~{\sf}~#1}}
\newcommand{\mytodogreen}[1]{\textcolor{mygreen}{\ding{46}~{\sf}~#1}}
\newcommand{\mytodoorange}[1]{\textcolor{orange}{\ding{46}~{\sf}~#1}}
\newcommand{\mytodocyan}[1]{\textcolor{cyan}{\ding{46}~{\sf}~#1}}
\newcommand{\mytodopink}[1]{\textcolor{purple}{\ding{46}~{\sf}~#1}}
\newcommand{\syn}[1]{\text{{\fontfamily{lmr}\selectfont{\small\textit{#1}}}}}
\newcommand{\tok}[1]{\text{{\fontfamily{lmr}\selectfont\small\textbf{#1}}}}
\newcommand{\scmd}[1]{\text{{\fontfamily{lmr}\selectfont\small\textcolor{gray}{#1}}}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{myhgreen}{#1}}
\newcommand{\gray}[1]{\textcolor{mgray}{#1}}

\newenvironment{lstcenter}[1][0.8\linewidth]
  {\begin{center}\begin{minipage}{#1}}
  {\end{minipage}\end{center}}

==> lib/todo-tags.tex <==
\usepackage{xcolor} 
\newif\ifshowtodos
\showtodostrue

\definecolor{turquoise}{RGB}{64,224,208}
\definecolor{darkteal}{RGB}{0,128,128}

\ifshowtodos
\newcommand{\ToResearch}[1]{\textcolor[RGB]{255,0,0}{[To Research: #1]}} \newcommand{\ToCite}[1]{\textcolor[RGB]{0,128,0}{[To Cite: #1]}} \newcommand{\ToRead}[1]{\textcolor[RGB]{0,0,255}{[To Read: #1]}} \newcommand{\ToWrite}[1]{\textcolor[RGB]{128,0,128}{[To Write: #1]}} \newcommand{\ToPreWork}[1]{\textcolor[RGB]{255,165,0}{[To PreWork: #1]}} \newcommand{\ToOpt}[1]{\textcolor[RGB]{255,20,147}{[To Opt: #1]}} \newcommand{\ToStartMyDay}[1]{\colorbox{darkteal}{\textcolor{white}{[To Start My Day: #1]}}}
\newcommand{\DateMark}[2]{\textcolor[RGB]{139,69,19}{[#1: #2]}} \newcommand{\ToAddInfo}[1]{\textcolor[RGB]{0,255,255}{[To Add Info: #1]}} \newcommand{\ToCheck}[1]{\textcolor[RGB]{255,191,0}{#1}} 
\newcommand{\ToThink}[1]{\textcolor[RGB]{173,216,230}{[To Think: #1]}} \else
\newcommand{\ToResearch}[1]{}
\newcommand{\ToCite}[1]{}
\newcommand{\ToRead}[1]{}
\newcommand{\ToWrite}[1]{}
\newcommand{\ToPreWork}[1]{}
\newcommand{\ToOpt}[1]{}
\newcommand{\ToStartMyDay}[1]{}
\newcommand{\ToThink}[1]{}
\newcommand{\DateMark}[2]{}
\newcommand{\ToAddInfo}[1]{}
\newcommand{\ToCheck}[1]{}
\fi

